Explosive Legged Robotic Hopping: Energy Accumulation and Power Amplification via Pneumatic Augmentation

We present a novel pneumatic augmentation to traditional electric motor-actuated legged robot to increase intermittent power density to perform infrequent explosive hopping behaviors. The pneumatic system is composed of a pneumatic pump, a tank, and a pneumatic actuator. The tank is charged up by the pump during regular hopping motion that is created by the electric motors. At any time after reaching a desired air pressure in the tank, a solenoid valve is utilized to rapidly release the air pressure to the pneumatic actuator (piston) which is used in conjunction with the electric motors to perform explosive hopping, increasing maximum hopping height for one or subsequent cycles. We show that, on a custom-designed one-legged hopping robot, without any additional power source and with this novel pneumatic augmentation system, their associated system identification and optimal control, the robot is able to realize highly explosive hopping with power amplification per cycle by a factor of approximately 5.4 times the power of electric motor actuation alone.

==> Xiaobin.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% anther possible layout: intro from hopping robots. 
%%% first paragraph: intro dynamic legged robots with good exmaple.
%%%%% motivate the hopping behaviors for locomtion: (hopping of singled legged robots) is cool because 
%%%numerate different robots 
%%% raibert, kod, ROBOTS with actuators, 
%%%%  

%% Yifei's intro version
% \input{yifei}
% \input{arturo}



%% legged robots -> one legged robots 
Legged robots, with the ability to make and break ground contact, select contact locations, and modulate gait are able to traverse a broader range of terrains than wheeled or tracked robots. They have shown great potentials in search and rescue \cite{bellicoso2018advances}, inspection \cite{gehring2021anymal}, and exploration in unstructured environments \cite{agha2021nebula}. Although legged robots can have different number of legs, joints, and morphologies, their locomotion behaviors are oftentimes cyclic, resulting the fact that negative work has to be performed in each cycle of the periodic motion. Taking hopping robots \cite{LeggedRobotThatBalance} as examples, before accelerating upwards to lift off the ground, the robots have to decelerate to a complete stop in the vertical direction in the descending phase by performing negative work to itself. 

%%% hopping behaviors, negative work-> elastic elements
%%%%%%%%%%% Problems with elastic elements, immediately release, 
%%%%%%%%%%%%% power output per hopping cycle is bounded 

Significant research activities in the literature have been focused on using elastic elements in the system to prevent using actuators to perform negative work for increasing energy efficiency and reducing the required actuator power in the design. The elastic elements are typically in the form of air springs \cite{LeggedRobotThatBalance} or mechanical springs \cite{grizzle2009mabel, brown1998bow, haldane2017repetitive, hubicki2016atrias, wang2023terrestrial}. The negative work in the descending phase can then be stored as spring potential energy and then return back to the system in the ascending phase of the cyclic motion. The springs are installed either in serial \cite{pratt1995series, yang2023small, EPA_hopper} or parallel \cite{Disney3D, 9636108} with the main actuators on the robots; despite this difference, the elastic energy has to be stored and release immediately within one cycle, which prevents the \textit{periodic energy accumulation for power amplification} to achieve subsequent emergent explosive maneuvers. 

 
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/Fig1_v6.png}
    \caption{The explosive jumping (right) that is "warmed up" by the regular periodic jumping behaviors (left) of the single legged hopping robot.}
    \label{fig:Robot design structure}
\end{figure}

 

%%%%%%%%%%%%%%%%%% We propose a design and control methodology that can storage energy lose during continuous operations, and produce infrequent high-power output motions as needed. 

To address this problem, we propose a design and control framework that augments legged robots with a pneumatic appendage to accumulate the energy of the negative work done in the locomotion cycles \textit{via a pump}, store it as air pressure \textit{in a tank}, and then exploit it \textit{through a pneumatic actuator} to perform subsequent high-power-output tasks that cannot be realized by the original motor actuation. The pneumatic appendage is installed in parallel with the original actuation so that the robot can perform regular motions and tasks as that without the pneumatic appendage. As negative work is to be performed in each locomotion cycle, the pump is actuated to push air into the tank which convert the negative work into air pressure to the tank. When the tank has stored enough air pressure, the pneumatic actuator can then be utilized in conjunction with the original actuator to amplify power output for explosive locomotion behaviors. 


%%% what we do in details  
We realize this framework on a single-legged hopping robot that is originally actuated only by electrical motors. We custom-design the pneumatic appendage based on the associated physical parameters of the robot. The control of hopping with the pneumatic appendage is rigorously realized via model-based techniques. With careful system identifications of the pneumatic system, its dynamics can be combined with canonical rigid-body dynamics model \cite{lynch2017modern} of the robot. We then use a direct collocation method \cite{hereid20163d, xiong2018bipedal, hubicki2016tractable} to optimize the trajectories for pneumatically-enhanced (and -enhanced-free) hopping behaviors based on a reduced order model. Task space position and force controls are deployed on the robot to realize these hopping behaviors. 

% and achived what
For this specific robot, we show that with the custom-design pneumatic appendage, the robot increases its hopping height from 1.8cm to 21cm, that is equivalently having a power amplification per cycle at 11.67. Moreover, the stored energy is shown to be utilized to perform challenging maneuvers, e.g., kicking a box over and then leaping on top of it, without additional power sources. \textbf{some more results here}. The results on the physical system validate our proposed approach, and furthermore indicate a promising design and control paradigm for power amplifications on highly dynamic legged robots.



==> arturo.tex <==
\par

The extent of the operation of an autonomous robot is limited by the energy stored in its batteries. Hopping robots based on linear springlike actuators can recapture and reuse some of the energy during each movement cycle. Current Hopping Robots designed for cyclic tasks include the storage of energy in spring actuators during the descent phase to be used to assist in the ascent phase to complete current operating cycle (step). 
 
To ensure walking robots can operate alongside humans in their environment or for disaster theaters where the terrain situation is changing constantly, the recapture and use of energy will likely require novel ways to capture and store energy to be used to extend the duration and types of tasks the autonomous hopping robot is expected to perform to achieve its mission.
 
The design proposed here uses a pneumatic assisted appendage that successfully harvests energy from the cyclic hopping tasks and store it in the form of air pressure to assist in, for example, power enhancement of current tasks or even more complex ones. The key contribution of this paper is a design framework without an external power source in the form of a pneumatic appendage enabling the manipulation of energy to amplify short term power to achieve enhanced (word) hopping.

Using a reduced order model of a single legged hopping robot as a basis, we performed trajectory optimization to get the force control and task space control profile for the cyclic and “enhanced” hopping. The pneumatic system introduces some non-linear constraints which drive the trajectory optimization problem into different stance phases. We experimentally validated the advantages of our framework design showing that a single legged hopping robot could achieve significantly higher jumps (over three times as high) with pneumatic augmentation than the electric motors could produce by themselves. 



==> michael.tex <==
Legged robots, with the ability to make and break ground contact, select contact locations, and modulate gait are able to traverse a broader range of terrains than wheeled or tracked robots. With potential applications in search and rescue, inspection, and exploration in unstructured environments, study of the underlying dynamics of legged robots is a compelling area of research [cite Raibert book and paper plus one more recent work by Professor Xiong]. 

Reducing the structure to a single leg allows detailed study of gait dynamics. these single-leg hoppers are often fixed to a gantry or boom system, 
%which constrains them to planar motion (or near planar curved motion) and allows the addition of a counterweight to modify the perceived weight of the robot [cite one or more early single legged hoppers with a boom]. 

%We divide hopping into two phases: 1. \textit{Aerial} phase no contact with ground and no Ground Reaction Force (GRF), and 2. \textit{Stance} phase, in which the foot of the device is in contact with the ground. Stance phase begins with a \textit{Descending} portion, during which the center of mass moves downward (actuators do negative work), followed by a \textit{Ascending} portion (actuators cause sufficient GRF to return the system to an aerial phase). 

To harness the energy absorbed during Descending, several hoppers have used springs or other elastic elements to store the energy absorbed during Descending, then release the energy during the Ascending portion of the following hop [SEA, Disney]. 
Others have explored the possibility of storing energy onboard in the form of compressed gas (CO2 canister) for infrequent very high leaps, with power densities far in excess of those capable with the motors alone [sand flea, Yifei’s citations].
In all of the described works, energy is either stored for a fraction of a gait cycle (elastic elements) or is preloaded on the robot (CO2 canister) and can not be recharged during operation. One recent work presented a spring-activated leaper, in which elastic rods were deflected by a motor (low power) then quickly released (high power) causing the device to leap to a great height. However, to achieve this leap, the system would stop, slowly deflect the rods, then leap. The high-power actuation could not be carried out during normal device operation.


%\textbf{[condense the literature review]} The field of legged robotics has long captivated researchers, driven by the ubiquity of legged animals in terrestrial environments. Unlike wheeled systems, which face limitations in varied terrain, legged robots boast the potential to traverse diverse landscapes. This capability positions them as invaluable assets in tasks ranging from search and rescue to industrial inspection and space exploration.
%While the broader field of legged robotics is vast, there is a particular interest in single-legged hopping robots. These robots, by avoiding the complexities inherent in multi-legged counterparts, offer a streamlined avenue for studying leg dynamics, stability, and control. What is particularly intriguing about single-legged hopping robots is their capability to traverse complex and uneven terrains with ease. This ability renders the specific shapes and sizes of obstacles and gaps insignificant for the robot's movement. This attribute not only holds immense research value but also promises significant real-world applications, marking a pivotal development in robotics.
%The evolution of hopping robots can be traced back to M.H. Raibert's pioneering work \cite{Raibert1984ExperimentsIB} \cite{Raibert3D}, which established the foundational principles of legged locomotion. Building upon Raibert's model, subsequent studies have explored various adaptations\cite{de_penn_2015}. Notably, Disney Research's LEAP robot represents a significant advancement in this domain. Incorporating a spring element into its design, LEAP aims to ensure safety in environments shared with humans by reducing the impact forces during hopping, thus demonstrating a critical balance between safety considerations and dynamic performance in robotic hopping. Others investigate alternative actuation mechanisms to store energy for better takeoff acceleration and energy efficiency performance\cite{Parallelelastic} \cite{salto} \cite{CableDriven}. For instance, UCSB's spring-actuated hopper achieved record heights but lacked dynamic motion control, with its energy storage and jumping cycles being disjointed. Pneumatically actuated hoppers have also been explored, delving into the nuanced interplay between motor control and morphological design \cite{Cham2001SeeLR} \cite{PneuHeightControl} \cite{PneuSlideControl}, particularly in robots with hybrid actuation systems combining electric motors and pneumatic artificial muscles (PAMs) \cite{EPA_hopper}.
%Previous research in legged robotics aiming for high jumps often relies on transient energy storage through elastic elements like springs within a gait cycle or employs external energy sources such as batteries or pre-charged compressed air for assistance. This approach often limits the autonomy and adaptability of the robots in dynamic environments. \textbf{(Move to later paragraph)} Our research addresses this gap by exploring a novel energy storage and utilization mechanism, harnessing mechanical energy conversion into pneumatic power, thereby enhancing the robot's operational efficiency and adaptability in real-world scenarios.

 
 
% Legged robots are cool
% Cyclic gaits
 %traverse more terrain than wheels or tracked 

% narrow to one leg
% brief lit review here 
 
%previous energy storage include battery which is charged beforehand, tank which is pressurized beforehand (or chemical), or a spring/elastic element which is "charged" during the descent of the gait, but used up immediately during the subsequent ascent 
%This is diff than ucsb spring
%%%% related work 
 %UCSB work compare: high jump but we want more control 
 %Jump had to be performed in isolation
%% DONT HAVE UCSB AS LAST THING IN 1 GOES ELSEWHERE

\
%%%% 2nd paragraph- GAP: itermediate high POWER density without high power actuator.   cost, weight,  
%%%% Among most of the legged hopping robots, the power density of the system is limited from the max power of actuator. It is however desired to achieve intermediate higher power density for infrequent tasks that requires high power density, e.g., high (?) jumping, kicking, 
%%%%%% 
% Power density is limited by actuators
% High power needed intermittently
 %         egs
 %storing energy in form of ... for use when needed

 
%\textbf{[sell the problem/state the gap]} The previously mentioned robots work well for periodic or cyclic tasks, but sometimes the need arises to perform a specialized task intermittently that requires more power/energy to complete, such as a higher jump or a kick. The robots previously discussed have a fixed power density determined by the electric actuators and any additional pre-included system. Therefore, the intermittent specialized task is limited by the parts selected for the robot. Furthermore, it is very uncommon for the pre-included system to be rechargeable during operation, and springs--while they do store some of the system's energy during the descent with each cycle--are incapable of saving energy for future use beyond the current period, specifically the grounded ascent phase. 
%% 

%% 3rd paragraph -- Our contribution
%% Desc our system ...
%\textbf{[Key Conceptual framework]} We valide the framework by designing a hopping robot with a pneumatic pump between the hip and foot which connects to a tank as a way to store energy in the form of pneumatic pressure. As the hopping robot performs its periodic gait, the pump compresses and adds pressure to the tank. The pressure in the tank can then be released at a later time into a pneumatic actuator mounted in parallel with the pump to complete an intermittent task that would require a higher energy input than the electric motors could provide by their lonesome. In order to achieve this, we modeled the dynamics of both moving components of the pneumatic system: the pump and the actuator. Using the approximate model, we implemented a novel control scheme to perform a pneumatically augmented hop. The key contributions of this work are integrating a regeneratable pneumatic system in parallel with a more traditional hopping robot, developing a model of the combined system, and performing simultaneous control of the combined subsystems to achieve a better performance than each individual subsystem could execute. 
We present a design methodology in which a legged robot stores energy during Descending but does not return the energy during the next hop (Fig. 1). Rather, the energy is stored in the form of compressed air in a tank for later use in infrequent high-power events during normal robot operation. We validate this methodology by appending a pneumatic system to a single-legged hopper. This hopper is able to store compressed gas to 340 kPa, increase leaping height from 1.8 cm to 21 cm, and perform maneuvers (kicking a box over then leaping on top of it), impossible using only its motors. \textit{The key contribution of this work} is a design framework adding pneumatic energy harvesting and storage to an electric-motor-based robot, to manipulate energy to amplify power short term without an additional power source. 


\textbf{[keyworkds: nonlinear trajectory optimization, reduced order model, force control, task space control.]}

\textbf{[key results:? performance ]}

The remainder of this paper is structured as follows. We first discuss the considerations taken when designing the system. We then examine the modeling of the pneumatic system and the hybrid dynamics of the combined system. We follow by elaborating on the control schema and trajectory optimization necessary to accomplish the periodic and intermittent tasks. Finally, we review the performance of the system. 

 %%Present approach for energy storage during performance of regular task
 %%Modeling and control (a couple sentences)
 %%"Key contributions of this work are" ...
%%%% hardware results 
 %% Increase power/etc. by x percent
 %%The remainder of this paper is structured as follows ... (Maybe not needed)

%%%%  Among most hopping robots, their 
%%%% second paragraph: increaing power density is challanging. (other exisiting trial solutions?)
 %%% talk about actuation 
%%%% thrid our approach 


==> yifei.tex <==
% introduction 
\par
Legged robotics has long captivated researchers, driven by the ability to traverse complex terrains than wheeled or tracked robots. With potential applications in search and rescue, inspection, and exploration in unstructured environments, study of underlying dynamics of legged robots is a compelling area of research. 



Considering complexities of legged robotic system, a lot of  researchers focus on  single-legged hopping robots, which first development by MIT/CMU Leg Laboratory \cite{LeggedRobotThatBalance}, including 2D and 3D hopper \cite{Raibert1984ExperimentsIB}\cite{Raibert3D}. These robot are highly dynamic platform that offers a streamlined avenue for studying leg dynamics and control problems. 

While hopping robots required significant force and speed to achieve notable height, demanding energy is needed for robot to lift-off the ground. One strategy is to utilize the energy absorbed during the impact between the robot and environment. Several hoppers have used elastic elements to store energy, like series elastic actuator (SEA) \cite{SeriesElasticActuator}  and parallel elastic actuator (PEA) \cite{Disney3D}.  Others have explored the possibility of storing energy on board in the form of compressed gas for hopping using its high power-to-weight ratio \cite{Cham2001SeeLR}\cite{PneuHeightControl}\cite{PneuSlideControl}. However, the studies mentioned above indicate that energy is either stored for only a fraction of a gait cycle or requires an additional energy source.
A recent study introduced a spring-activated hopper that attained record heights with isolated energy storage and release process  \cite{UCSBHighest} but this system lacks controllability during normal operations.

\par
Existing hopping robots excel in repetitive tasks but lack the capacity for high-power actions like executing a higher jump. This limitation stems from their fixed power output dictated by the actuator. Furthermore, while some robots use springs or other means to temporarily store energy, they lack the ability to accumulate and utilize this energy over multiple jumping cycles. This limitation becomes particularly evident in tasks that require sudden bursts of energy beyond their standard operational capacity. Our research addresses this challenge, offering a solution that enhances energy storage and utilization across multiple cycles.

